DeepSync: A Learning Framework for Pervasive Localization using Code Synchronization on Compressed Cellular Spectrum

Pervasive localization is essential for continuous tracking applications, yet existing solutions face challenges in balancing power consumption and accuracy. GPS, while precise, is impractical for continuous tracking of micro-assets due to high power requirements. Recent advances in non-linear compressed spectrum sensing offer low-power alternatives, but existing implementations achieve only coarse positioning through Received Signal Strength Indicator (RSSI) measurements. We present DeepSync, a deep learning framework that enables precise localization using compressed cellular spectrum. Our key technical insight lies in formulating sub-sample timing estimation as a template matching problem, solved through a novel architecture combining temporal CNN encoders for multi-frame processing with cross-attention mechanisms. The system processes non-linear inter-modulated spectrum through hierarchical feature extraction, achieving robust performance at SNR levels below -10dB -- a regime where conventional timing estimation fails. By integrating real cellular infrastructure data with physics-based ray-tracing simulations, DeepSync achieves 2.128-meter median accuracy while consuming significantly less power than conventional systems. Real-world evaluations demonstrate 10x improvement over existing compressed spectrum approaches, establishing a new paradigm for ultra-low-power localization.

==> backup_citations.tex <==
@misc{sectorizedcell,
	key = {SEQUANS},
	title = {LTE Network Design},
	howpublished={Online:\\ \url{https://lteanddrones.com/2-lte-network-design#:~:text=In%20an%20LTE%20cellular%20network,not%20interfere%20with%20each%20other}},
	note = {Accessed on January 29, 2023}
}
@misc{ltebands,
	key = {lte bands},
	title = {LTE frequency bands},
	howpublished={Online:\\ \url{https://en.wikipedia.org/wiki/LTE_frequency_bands}},
	note = {Accessed on January 29, 2023}
}
@article{malekzadeh20193,
  title={3-sector cell vs. omnicell: Cell sectorization impact on the performance of side-by-side unlicensed lte and 802.11 ac air interfaces},
  author={Malekzadeh, Mina and Ghani, Abdul Azim Abdul},
  journal={IEEE Access},
  volume={7},
  pages={122315--122329},
  year={2019},
  publisher={IEEE}
}
@misc{usabands,
	key = {USA bands},
	title = {LTE frequency bands list for Mobile Carriers : US and Canada Guide},
	howpublished={Online:\\ \url{https://www.myamplifiers.com/articles/lte-frequency-bands-of-us-and-canada-carriers/}},
	note = {Accessed on January 29, 2023}
}
@misc{contdownlink,
	key = {LTE PHY},
	title = {White paper: Long Term Evolution Protocol Overview},
	howpublished={Online:\\ \url{https://www.nxp.com/docs/en/white-paper/LTEPTCLOVWWP.pdf}},
	note = {Accessed on January 30, 2023}
}
@misc{ofdmperslot,
	key = {LTE frame structure},
	title = {LTE Slot Structure},
	howpublished={Online:\\ \url{https://www.ni.com/docs/en-US/bundle/rfmx-waveform-creator/page/lte-slot-structure.html}},
	note = {Accessed on January 30, 2023}
}




@inproceedings{elbakly2019crescendo,
  title={Crescendo: An infrastructure-free ubiquitous cellular network-based localization system},
  author={Elbakly, Rizanne and Youssef, Moustafa},
  booktitle={2019 IEEE Wireless Communications and Networking Conference (WCNC)},
  pages={1--6},
  year={2019},
  organization={IEEE}
}


@article{won2020three,
  title={Three decades of 3GPP target cell search through 3G, 4G, and 5G},
  author={Won, Seunghwan and Choi, Sang Won},
  journal={IEEE Access},
  volume={8},
  pages={116914--116960},
  year={2020},
  publisher={IEEE}
}
%
%@article{cui2003autonomous,
%  title={Autonomous vehicle positioning with GPS in urban canyon environments},
%  author={Cui, Youjing and Ge, Shuzhi Sam},
%  journal={IEEE transactions on robotics and automation},
%  volume={19},
%  number={1},
%  pages={15--25},
%  year={2003},
%  publisher={IEEE}
%}
%
%
%@misc{,
%  author =       "Name",
%  year =         "2023",
%  howpublished = "\url{}",
%}
%
%@misc{fccreport,
%  author =       "FCC",
%  year =         "2023",
%  howpublished = "\url{https://docs.fcc.gov/public/attachments/DA-15-1487A1.pdf}",
%}
%
%@misc{raspberrypi,
%  author =       "Raspberry Pi",
%  year =         "2023",
%  howpublished = "\url{https://www.raspberrypi.com/products/raspberry-pi-3-model-b/}",
%}
%
%@misc{intelrealsense,
%  author =       "Intel",
%  year =         "2023",
%  howpublished = "\url{https://dev.intelrealsense.com/docs/tracking-camera-t265-datasheet}",
%}
%
%@misc{muratauwb,
%  author =       "Murata",
%  year =         "2023",
%  howpublished = "\url{https://www.murata.com/en-us/products/connectivitymodule/ultra-wide-band/nxp/type2bp}",
%}
%
%
%@misc{viconv8,
%  author =       "Vicon",
%  year =         "2023",
%  howpublished = "\url{https://docs.vicon.com/display/Vantage/V8+camera+specifications}",
%}
%
%@inproceedings{di2017calibration,
%  title={Calibration-free network localization using non-line-of-sight ultra-wideband measurements},
%  author={Di Franco, Carmelo and Prorok, Amanda and Atanasov, Nikolay and Kempke, Benjamin and Dutta, Prabal and Kumar, Vijay and Pappas, George J},
%  booktitle={Proceedings of the 16th ACM/IEEE International Conference on Information Processing in Sensor Networks},
%  pages={235--246},
%  year={2017}
%}
%
%@inproceedings{miller2022cappella,
%  title={Cappella: Establishing Multi-User Augmented Reality Sessions Using Inertial Estimates and Peer-to-Peer Ranging},
%  author={Miller, John and Soltanaghai, Elahe and Duvall, Raewyn and Chen, Jeff and Bhat, Vikram and Pereira, Nuno and Rowe, Anthony},
%  booktitle={2022 21st ACM/IEEE International Conference on Information Processing in Sensor Networks (IPSN)},
%  pages={428--440},
%  year={2022},
%  organization={IEEE}
%}
%
%@inproceedings{klopschitz2007automatic,
%  title={Automatic reconstruction of wide-area fiducial marker models},
%  author={Klopschitz, Manfred and Schmalstieg, Dieter},
%  booktitle={2007 6th IEEE and ACM International Symposium on Mixed and Augmented Reality},
%  pages={71--74},
%  year={2007},
%  organization={IEEE}
%}
%
%@inproceedings{mulloni2011handheld,
%  title={Handheld augmented reality indoor navigation with activity-based instructions},
%  author={Mulloni, Alessandro and Seichter, Hartmut and Schmalstieg, Dieter},
%  booktitle={Proceedings of the 13th international conference on human computer interaction with mobile devices and services},
%  pages={211--220},
%  year={2011}
%}
%
%@inproceedings{kallwies2020determining,
%  title={Determining and improving the localization accuracy of AprilTag detection},
%  author={Kallwies, Jan and Forkel, Bianca and Wuensche, Hans-Joachim},
%  booktitle={2020 IEEE International Conference on Robotics and Automation (ICRA)},
%  pages={8288--8294},
%  year={2020},
%  organization={IEEE}
%}
%
%@inproceedings{wang2016apriltag,
%  title={AprilTag 2: Efficient and robust fiducial detection},
%  author={Wang, John and Olson, Edwin},
%  booktitle={2016 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
%  pages={4193--4198},
%  year={2016},
%  organization={IEEE}
%}
%
%@inproceedings{zhao2020relative,
%  title={Relative Localization for UAVs Based on April-Tags},
%  author={Zhao, Boxin and Li, Zongzhe and Jiang, Jun and Zhao, Xiaolin},
%  booktitle={2020 Chinese Control And Decision Conference (CCDC)},
%  pages={444--449},
%  year={2020},
%  organization={IEEE}
%}
%
%@article{nguyen2021range,
%  title={Range-focused fusion of camera-IMU-UWB for accurate and drift-reduced localization},
%  author={Nguyen, Thien Hoang and Nguyen, Thien-Minh and Xie, Lihua},
%  journal={IEEE Robotics and Automation Letters},
%  volume={6},
%  number={2},
%  pages={1678--1685},
%  year={2021},
%  publisher={IEEE}
%}
%
%@inproceedings{olsson2014cooperative,
%  title={Cooperative localization using a foot-mounted inertial navigation system and ultrawideband ranging},
%  author={Olsson, Fredrik and Rantakokko, Jouni and Nyg{\aa}rds, Jonas},
%  booktitle={2014 International conference on indoor positioning and indoor navigation (IPIN)},
%  pages={122--131},
%  year={2014},
%  organization={IEEE}
%}
%
%@article{shule2020uwb,
%  title={Uwb-based localization for multi-uav systems and collaborative heterogeneous multi-robot systems},
%  author={Shule, Wang and Almansa, Carmen Mart{\'\i}nez and Queralta, Jorge Pe{\~n}a and Zou, Zhuo and Westerlund, Tomi},
%  journal={Procedia Computer Science},
%  volume={175},
%  pages={357--364},
%  year={2020},
%  publisher={Elsevier}
%}
%
%@article{vcapkun2002gps,
%  title={GPS-free positioning in mobile ad hoc networks},
%  author={{\v{C}}apkun, Srdjan and Hamdi, Maher and Hubaux, Jean-Pierre},
%  journal={Cluster Computing},
%  volume={5},
%  pages={157--167},
%  year={2002},
%  publisher={Springer}
%}
%
%@inproceedings{shao2018marble,
%  title={Marble: Mobile augmented reality using a distributed ble beacon infrastructure},
%  author={Shao, Chong and Islam, Bashima and Nirjon, Shahriar},
%  booktitle={2018 IEEE/ACM Third International Conference on Internet-of-Things Design and Implementation (IoTDI)},
%  pages={60--71},
%  year={2018},
%  organization={IEEE}
%}
%
%@inproceedings{gomez2013indoor,
%  title={Indoor augmented reality based on ultrasound localization systems},
%  author={G{\'o}mez, David and Tarr{\'\i}o, Paula and Li, Juan and Bernardos, Ana M and Casar, Jos{\'e} R},
%  booktitle={Highlights on Practical Applications of Agents and Multi-Agent Systems: International Workshops of PAAMS 2013, Salamanca, Spain, May 22-24, 2013. Proceedings 11},
%  pages={202--212},
%  year={2013},
%  organization={Springer}
%}
%
%@inproceedings{lazik2015alps,
%  title={ALPS: A bluetooth and ultrasound platform for mapping and localization},
%  author={Lazik, Patrick and Rajagopal, Niranjini and Shih, Oliver and Sinopoli, Bruno and Rowe, Anthony},
%  booktitle={Proceedings of the 13th ACM conference on embedded networked sensor systems},
%  pages={73--84},
%  year={2015}
%}
%
%@inproceedings{li2018automatic,
%  title={An automatic and accurate localization system for firefighters},
%  author={Li, Jinyang and Xie, Zhiheng and Sun, Xiaoshan and Tang, Jian and Liu, Hengchang and Stankovic, John A},
%  booktitle={2018 IEEE/ACM Third International Conference on Internet-of-Things Design and Implementation (IoTDI)},
%  pages={13--24},
%  year={2018},
%  organization={IEEE}
%}
%
%@inproceedings{dhekne2019trackio,
%  title={TrackIO: Tracking First Responders Inside-Out.},
%  author={Dhekne, Ashutosh and Chakraborty, Ayon and Sundaresan, Karthikeyan and Rangarajan, Sampath},
%  booktitle={NSDI},
%  volume={19},
%  pages={751--764},
%  year={2019}
%}
%
%@inproceedings{gentner2017simultaneous,
%  title={Simultaneous localization and mapping for pedestrians using low-cost ultra-wideband system and gyroscope},
%  author={Gentner, Christian and Ulmschneider, Markus},
%  booktitle={2017 International Conference on Indoor Positioning and Indoor Navigation (IPIN)},
%  pages={1--8},
%  year={2017},
%  organization={IEEE}
%}
%
%@inproceedings{liu2017cooperative,
%  title={Cooperative relative positioning of mobile users by fusing IMU inertial and UWB ranging information},
%  author={Liu, Ran and Yuen, Chau and Do, Tri-Nhut and Jiao, Dewei and Liu, Xiang and Tan, U-Xuan},
%  booktitle={2017 IEEE International Conference on Robotics and Automation (ICRA)},
%  pages={5623--5629},
%  year={2017},
%  organization={IEEE}
%}
%
%@inproceedings{rajagopal2019improving,
%  title={Improving augmented reality relocalization using beacons and magnetic field maps},
%  author={Rajagopal, Niranjini and Miller, John and Kumar, Krishna Kumar Reghu and Luong, Anh and Rowe, Anthony},
%  booktitle={2019 International Conference on Indoor Positioning and Indoor Navigation (IPIN)},
%  pages={1--8},
%  year={2019},
%  organization={IEEE}
%}
%
%@inproceedings{song2019uwb,
%  title={Uwb/lidar fusion for cooperative range-only slam},
%  author={Song, Yang and Guan, Mingyang and Tay, Wee Peng and Law, Choi Look and Wen, Changyun},
%  booktitle={2019 international conference on robotics and automation (ICRA)},
%  pages={6568--6574},
%  year={2019},
%  organization={IEEE}
%}
%
%@inproceedings{wang2017ultra,
%  title={Ultra-wideband aided fast localization and mapping system},
%  author={Wang, Chen and Zhang, Handuo and Nguyen, Thien-Minh and Xie, Lihua},
%  booktitle={2017 IEEE/RSJ international conference on intelligent robots and systems (IROS)},
%  pages={1602--1609},
%  year={2017},
%  organization={IEEE}
%}
%
%@inproceedings{nagpal2003organizing,
%  title={Organizing a global coordinate system from local information on an ad hoc sensor network},
%  author={Nagpal, Radhika and Shrobe, Howard and Bachrach, Jonathan},
%  booktitle={Information Processing in Sensor Networks: Second International Workshop, IPSN 2003, Palo Alto, CA, USA, April 22--23, 2003 Proceedings},
%  pages={333--348},
%  year={2003},
%  organization={Springer}
%}
%
%@inproceedings{savvides2001dynamic,
%  title={Dynamic fine-grained localization in ad-hoc networks of sensors},
%  author={Savvides, Andreas and Han, Chih-Chieh and Strivastava, Mani B},
%  booktitle={Proceedings of the 7th annual international conference on Mobile computing and networking},
%  pages={166--179},
%  year={2001}
%}
%
%@inproceedings{eren2004rigidity,
%  title={Rigidity, computation, and randomization in network localization},
%  author={Eren, Tolga and Goldenberg, OK and Whiteley, Walter and Yang, Yang Richard and Morse, A Stephen and Anderson, Brian DO and Belhumeur, Peter N},
%  booktitle={IEEE INFOCOM 2004},
%  volume={4},
%  pages={2673--2684},
%  year={2004},
%  organization={IEEE}
%}
%
%@inproceedings{moore2004robust,
%  title={Robust distributed network localization with noisy range measurements},
%  author={Moore, David and Leonard, John and Rus, Daniela and Teller, Seth},
%  booktitle={Proceedings of the 2nd international conference on Embedded networked sensor systems},
%  pages={50--61},
%  year={2004}
%}
%
%@inproceedings{rad2011cooperative,
%  title={Cooperative mobile network localization via subspace tracking},
%  author={Rad, Hadi Jamali and Amar, Alon and Leus, Geert},
%  booktitle={2011 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
%  pages={2612--2615},
%  year={2011},
%  organization={IEEE}
%}
%
%@inproceedings{nguyen2020vision,
%  title={Vision-based multi-MAV localization with anonymous relative measurements using coupled probabilistic data association filter},
%  author={Nguyen, Ty and Mohta, Kartik and Taylor, Camillo J and Kumar, Vijay},
%  booktitle={2020 IEEE International Conference on Robotics and Automation (ICRA)},
%  pages={3349--3355},
%  year={2020},
%  organization={IEEE}
%}
%
%@article{walter2019uvdar,
%  title={Uvdar system for visual relative localization with application to leader--follower formations of multirotor uavs},
%  author={Walter, Viktor and Staub, Nicolas and Franchi, Antonio and Saska, Martin},
%  journal={IEEE Robotics and Automation Letters},
%  volume={4},
%  number={3},
%  pages={2637--2644},
%  year={2019},
%  publisher={IEEE}
%}
%
%@article{ziegler2021distributed,
%  title={Distributed formation estimation via pairwise distance measurements},
%  author={Ziegler, Thomas and Karrer, Marco and Schmuck, Patrik and Chli, Margarita},
%  journal={IEEE Robotics and Automation Letters},
%  volume={6},
%  number={2},
%  pages={3017--3024},
%  year={2021},
%  publisher={IEEE}
%}
%
%@article{bai2020high,
%  title={A high-precision and low-cost IMU-based indoor pedestrian positioning technique},
%  author={Bai, Nan and Tian, Yuan and Liu, Ye and Yuan, Zhengxi and Xiao, Zhuoling and Zhou, Jun},
%  journal={IEEE Sensors Journal},
%  volume={20},
%  number={12},
%  pages={6716--6726},
%  year={2020},
%  publisher={IEEE}
%}
%
%@inproceedings{cao2021relative,
%  title={Relative localization of mobile robots with multiple ultra-wideband ranging measurements},
%  author={Cao, Zhiqiang and Liu, Ran and Yuen, Chau and Athukorala, Achala and Ng, Benny Kai Kiat and Mathanraj, Muraleetharan and Tan, U-Xuan},
%  booktitle={2021 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
%  pages={5857--5863},
%  year={2021},
%  organization={IEEE}
%}
%
%@article{guo2019ultra,
%  title={Ultra-wideband and odometry-based cooperative relative localization with application to multi-UAV formation control},
%  author={Guo, Kexin and Li, Xiuxian and Xie, Lihua},
%  journal={IEEE transactions on cybernetics},
%  volume={50},
%  number={6},
%  pages={2590--2603},
%  year={2019},
%  publisher={IEEE}
%}
%
%@article{guo2017ultra,
%  title={Ultra-wideband based cooperative relative localization algorithm and experiments for multiple unmanned aerial vehicles in GPS denied environments},
%  author={Guo, Kexin and Qiu, Zhirong and Meng, Wei and Xie, Lihua and Teo, Rodney},
%  journal={International Journal of Micro Air Vehicles},
%  volume={9},
%  number={3},
%  pages={169--186},
%  year={2017},
%  publisher={SAGE Publications Sage UK: London, England}
%}
%
%@inproceedings{li2020relative,
%  title={Relative localization in multi-robot systems based on dead reckoning and uwb ranging},
%  author={Li, Ming and Chang, Zhuang and Zhong, Zhen and Gao, Yan},
%  booktitle={2020 IEEE 23rd International Conference on Information Fusion (FUSION)},
%  pages={1--7},
%  year={2020},
%  organization={IEEE}
%}
%
%@article{xu2022omni,
%  title={Omni-Swarm: A Decentralized Omnidirectional Visual--Inertial--UWB State Estimation System for Aerial Swarms},
%  author={Xu, Hao and Zhang, Yichen and Zhou, Boyu and Wang, Luqi and Yao, Xinjie and Meng, Guotao and Shen, Shaojie},
%  journal={IEEE Transactions on Robotics},
%  volume={38},
%  number={6},
%  pages={3374--3394},
%  year={2022},
%  publisher={IEEE}
%}
%
%@inproceedings{xu2020decentralized,
%  title={Decentralized visual-inertial-uwb fusion for relative state estimation of aerial swarm},
%  author={Xu, Hao and Wang, Luqi and Zhang, Yichen and Qiu, Kejie and Shen, Shaojie},
%  booktitle={2020 IEEE international conference on robotics and automation (ICRA)},
%  pages={8776--8782},
%  year={2020},
%  organization={IEEE}
%}
%
%@misc{optitrack,
% title={OptiTrack},
% howpublished = "\url{https://optitrack.com/}",
% journal={OptiTrack},
% note = "Last accessed 12 March 2023"
%}
%
%@misc{vicon,
% title={Vicon},
% howpublished = "\url{https://www.vicon.com/}",
% journal={Vicon},
% note = "Last accessed 12 March 2023"
%}
%
%@INPROCEEDINGS{5940633,
%  author={Taris, T. and Begueret, JB. and Deval, Y.},
%  booktitle={2011 IEEE Radio Frequency Integrated Circuits Symposium}, 
%  title={A 60µW LNA for 2.4 GHz wireless sensors network applications}, 
%  year={2011},
%  volume={},
%  number={},
%  pages={1-4},
%  doi={10.1109/RFIC.2011.5940633}}
%@misc{HSMS285x,
%  author = "Hewlett-Packards",
%
%  howpublished = "\url{https://www.hpl.hp.com/hpjournal/95dec/dec95a12.pdf}",
%}
%@INPROCEEDINGS{4523148,
%  author={van Elzakker, Michiel and van Tuijl, Ed and Geraedts, Paul and Schinkel, Daniel and Klumperink, Eric and Nauta, Bram},
%  booktitle={2008 IEEE International Solid-State Circuits Conference - Digest of Technical Papers}, 
%  title={A 1.9μW 4.4fJ/Conversion-step 10b 1MS/s Charge-Redistribution ADC}, 
%  year={2008},
%  volume={},
%  number={},
%  pages={244-610},
%  doi={10.1109/ISSCC.2008.4523148}}


@article{bouten2013flexible,
  title={A flexible GPS tracking system for studying bird behaviour at multiple scales},
  author={Bouten, Willem and Baaij, Edwin W and Shamoun-Baranes, Judy and Camphuysen, Kees CJ},
  journal={Journal of Ornithology},
  volume={154},
  pages={571--580},
  year={2013},
  publisher={Springer}
}

@inproceedings{kim2009sss,
  title={SSS detection method for initial cell search in 3GPP LTE FDD/TDD dual mode receiver},
  author={Kim, Jung-In and Han, Jung-Su and Roh, Hee-Jin and Choi, Hyung-Jin},
  booktitle={2009 9th International Symposium on Communications and Information Technology},
  pages={199--203},
  year={2009},
  organization={IEEE}
}

@inproceedings{yang2011pss,
  title={PSS based time synchronization for 3GPP LTE downlink receivers},
  author={Yang, Xiumei and Xiong, Yong and Jia, Guoqing and Fang, Weidong and Zheng, Xiaoying},
  booktitle={2011 IEEE 13th International Conference on Communication Technology},
  pages={930--933},
  year={2011},
  organization={IEEE}
}

@inproceedings{wu2010physical,
  title={Physical cell identity self-organization for home eNodeB deployment in LTE},
  author={Wu, Yi and Jiang, Hai and Wu, Ye and Zhang, Dongmei},
  booktitle={2010 6th International Conference on Wireless Communications Networking and Mobile Computing (WiCOM)},
  pages={1--6},
  year={2010},
  organization={IEEE}
}

@article{evenson2015systematic,
  title={Systematic review of the validity and reliability of consumer-wearable activity trackers},
  author={Evenson, Kelly R and Goto, Michelle M and Furberg, Robert D},
  journal={International Journal of Behavioral Nutrition and Physical Activity},
  volume={12},
  number={1},
  pages={1--22},
  year={2015},
  publisher={BioMed Central}
}

@article{del2017survey,
  title={Survey of cellular mobile radio localization methods: From 1G to 5G},
  author={del Peral-Rosado, Jos{\'e} A and Raulefs, Ronald and L{\'o}pez-Salcedo, Jos{\'e} A and Seco-Granados, Gonzalo},
  journal={IEEE Communications Surveys \& Tutorials},
  volume={20},
  number={2},
  pages={1124--1148},
  year={2017},
  publisher={IEEE}
}

@article{hassija2020survey,
  title={A survey on supply chain security: Application areas, security threats, and solution architectures},
  author={Hassija, Vikas and Chamola, Vinay and Gupta, Vatsal and Jain, Sarthak and Guizani, Nadra},
  journal={IEEE Internet of Things Journal},
  volume={8},
  number={8},
  pages={6222--6246},
  year={2020},
  publisher={IEEE}
}

@article{willis2004evaluating,
  title={Evaluating the security of the global containerized supply chain},
  author={Willis, Henry H and Ortiz, David Santana},
  year={2004},
  publisher={Rand Corporation Santa Monica, CA}
}

@inproceedings{gadre2020frequency,
  title={Frequency Configuration for $\{$Low-Power$\}$$\{$Wide-Area$\}$ Networks in a Heartbeat},
  author={Gadre, Akshay and Narayanan, Revathy and Luong, Anh and Rowe, Anthony and Iannucci, Bob and Kumar, Swarun},
  booktitle={17th USENIX Symposium on Networked Systems Design and Implementation (NSDI 20)},
  pages={339--352},
  year={2020}
}

@inproceedings{bansal2021owll,
  title={Owll: Accurate lora localization using the tv whitespaces},
  author={Bansal, Atul and Gadre, Akshay and Singh, Vaibhav and Rowe, Anthony and Iannucci, Bob and Kumar, Swarun},
  booktitle={Proceedings of the 20th International Conference on Information Processing in Sensor Networks (co-located with CPS-IoT Week 2021)},
  pages={148--162},
  year={2021}
}

@misc{EnergyTrace,
  author =       "TI",
  title={Texas Instruments EnergyTrace++},
  year =         "2024",
  howpublished = "\url{https://www.ti.com/tool/ENERGYTRACE}",
}

@misc{3gpp25,
  author =       "3GPP",
  title = {Physical Layer Procedures (FDD), document 3GPP TS 25.214 v(12.3.0)},
  year =         "2024",
  howpublished = "\url{https://www.etsi.org/deliver/etsi_ts/125200_125299/125214/11.03.00_60/ts_125214v110300p.pdf}",
}

@article{won2020three,
  title={Three decades of 3GPP target cell search through 3G, 4G, and 5G},
  author={Won, Seunghwan and Choi, Sang Won},
  journal={IEEE Access},
  volume={8},
  pages={116914--116960},
  year={2020},
  publisher={IEEE}
}

@inproceedings{jog2022enabling,
  title={Enabling $\{$IoT$\}$$\{$Self-Localization$\}$ Using Ambient 5G Signals},
  author={Jog, Suraj and Guan, Junfeng and Madani, Sohrab and Lu, Ruochen and Gong, Songbin and Vasisht, Deepak and Hassanieh, Haitham},
  booktitle={19th USENIX Symposium on Networked Systems Design and Implementation (NSDI 22)},
  pages={1011--1026},
  year={2022}
}

@article{hassaniehghz,
  title={GHz-Wide Spectrum Sensing and Decoding},
  author={Hassanieh, Haitham}
}

@inproceedings{guddeti2019sweepsense,
  title={$\{$SweepSense$\}$: Sensing 5 $\{$GHz$\}$ in 5 Milliseconds with Low-cost Radios},
  author={Guddeti, Yeswanth and Subbaraman, Raghav and Khazraee, Moein and Schulman, Aaron and Bharadia, Dinesh},
  booktitle={16th USENIX Symposium on Networked Systems Design and Implementation (NSDI 19)},
  pages={317--330},
  year={2019}
}

@inproceedings{subbaraman2023crescendo,
  title={Crescendo: Towards Wideband, Real-Time, High-Fidelity Spectrum Sensing Systems},
  author={Subbaraman, Raghav and Mills, Kevin and Schulman, Aaron and Bharadia, Dinesh},
  booktitle={Proceedings of the 29th Annual International Conference on Mobile Computing and Networking},
  pages={1--14},
  year={2023}
}

@misc{signalhound,
  author =       "Signal Hound",
  title = {SM200C - 20 GHz Real-time Spectrum An- alyzer with 10GbE},
  year =         "2024",
  howpublished = "\url{https://signalhound.com/products/sm200c-20-ghz-real-time-spectrum-analyzer-with-10gbe/}",
}

@inproceedings{nandakumar2016fingerio,
  title={Fingerio: Using active sonar for fine-grained finger tracking},
  author={Nandakumar, Rajalakshmi and Iyer, Vikram and Tan, Desney and Gollakota, Shyamnath},
  booktitle={Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems},
  pages={1515--1525},
  year={2016}
}

@inproceedings{vasisht2016decimeter,
  title={$\{$Decimeter-Level$\}$ localization with a single $\{$WiFi$\}$ access point},
  author={Vasisht, Deepak and Kumar, Swarun and Katabi, Dina},
  booktitle={13th USENIX Symposium on Networked Systems Design and Implementation (NSDI 16)},
  pages={165--178},
  year={2016}
}

@article{choi2005blind,
  title={Blind source separation and independent component analysis: A review},
  author={Choi, Seungjin and Cichocki, Andrzej and Park, Hyung-Min and Lee, Soo-Young},
  journal={Neural Information Processing-Letters and Reviews},
  volume={6},
  number={1},
  pages={1--57},
  year={2005}
}


@misc{mozillalocation,
  author =       "Mozilla",
  title = {Mozilla Location Services},
  year =         "2024",
  howpublished = "\url{https://location.services.mozilla.com}",
}

@misc{cellmapper,
  author =       "CellMapper",
  title = {CellMapper},
  year =         "2024",
  howpublished = "\url{https://www.cellmapper.net/}",
}


@misc{opencellid,
  author =       "Open Cell ID",
  title = {Open Cell ID},
  year =         "2024",
  howpublished = "\url{https://opencellid.org/}",
}

@misc{msp430,
  author =       "Texas Instruments",
  year =         "2024",
  howpublished = "\url{https://www.ti.com/tool/MSP-EXP430FR5969}",
}

@inproceedings{rostami2021mixiq,
  title={MIXIQ: re-thinking ultra-low power receiver design for next-generation on-body applications},
  author={Rostami, Mohammad and Chen, Xingda and Feng, Yuda and Sundaresan, Karthikeyan and Ganesan, Deepak},
  booktitle={Proceedings of the 27th Annual International Conference on Mobile Computing and Networking},
  pages={364--377},
  year={2021}
}

@inproceedings{wentzloff2020ultra,
  title={Ultra-low power receivers for IoT applications: A review},
  author={Wentzloff, David D and Alghaihab, Abdullah and Im, Jaeho},
  booktitle={2020 IEEE Custom Integrated Circuits Conference (CICC)},
  pages={1--8},
  year={2020},
  organization={IEEE}
}

@misc{sms7630,
  author =       "Skyworks",
  year =         "2024",
  howpublished = "\url{https://store.skyworksinc.com/products/detail/sms7630006-skyworks/150612/}",
}

@misc{googleroadinspector,
   author = {{Google}},
   title = {{Google Road Inspector}},
   howpublished = "\url{https://developers.google.com/maps/documentation/roads/inspector}",
   year = {2024},
 }

@misc{tagolasantenna,
   author = {{tagolas}},
   title = {{Tagolas antenna}},
   howpublished = "\url{https://www.taoglas.com/datasheets/TG.22.0221.pdf}",
   year = {2024},
 }

@inproceedings{elbakly2019crescendo,
  title={Crescendo: An infrastructure-free ubiquitous cellular network-based localization system},
  author={Elbakly, Rizanne and Youssef, Moustafa},
  booktitle={2019 IEEE Wireless Communications and Networking Conference (WCNC)},
  pages={1--6},
  year={2019},
  organization={IEEE}
}


@article{won2020three,
  title={Three decades of 3GPP target cell search through 3G, 4G, and 5G},
  author={Won, Seunghwan and Choi, Sang Won},
  journal={IEEE Access},
  volume={8},
  pages={116914--116960},
  year={2020},
  publisher={IEEE}
}

@article{cui2003autonomous,
  title={Autonomous vehicle positioning with GPS in urban canyon environments},
  author={Cui, Youjing and Ge, Shuzhi Sam},
  journal={IEEE transactions on robotics and automation},
  volume={19},
  number={1},
  pages={15--25},
  year={2003},
  publisher={IEEE}
}


@misc{,
  author =       "Name",
  year =         "2023",
  howpublished = "\url{}",
}

@misc{fccreport,
  author =       "FCC",
  year =         "2023",
  howpublished = "\url{https://docs.fcc.gov/public/attachments/DA-15-1487A1.pdf}",
}

@misc{raspberrypi,
  author =       "Raspberry Pi",
  year =         "2023",
  howpublished = "\url{https://www.raspberrypi.com/products/raspberry-pi-3-model-b/}",
}

@misc{intelrealsense,
  author =       "Intel",
  year =         "2023",
  howpublished = "\url{https://dev.intelrealsense.com/docs/tracking-camera-t265-datasheet}",
}

@misc{muratauwb,
  author =       "Murata",
  year =         "2023",
  howpublished = "\url{https://www.murata.com/en-us/products/connectivitymodule/ultra-wide-band/nxp/type2bp}",
}


@misc{viconv8,
  author =       "Vicon",
  year =         "2023",
  howpublished = "\url{https://docs.vicon.com/display/Vantage/V8+camera+specifications}",
}

@inproceedings{di2017calibration,
  title={Calibration-free network localization using non-line-of-sight ultra-wideband measurements},
  author={Di Franco, Carmelo and Prorok, Amanda and Atanasov, Nikolay and Kempke, Benjamin and Dutta, Prabal and Kumar, Vijay and Pappas, George J},
  booktitle={Proceedings of the 16th ACM/IEEE International Conference on Information Processing in Sensor Networks},
  pages={235--246},
  year={2017}
}

@inproceedings{miller2022cappella,
  title={Cappella: Establishing Multi-User Augmented Reality Sessions Using Inertial Estimates and Peer-to-Peer Ranging},
  author={Miller, John and Soltanaghai, Elahe and Duvall, Raewyn and Chen, Jeff and Bhat, Vikram and Pereira, Nuno and Rowe, Anthony},
  booktitle={2022 21st ACM/IEEE International Conference on Information Processing in Sensor Networks (IPSN)},
  pages={428--440},
  year={2022},
  organization={IEEE}
}

@inproceedings{klopschitz2007automatic,
  title={Automatic reconstruction of wide-area fiducial marker models},
  author={Klopschitz, Manfred and Schmalstieg, Dieter},
  booktitle={2007 6th IEEE and ACM International Symposium on Mixed and Augmented Reality},
  pages={71--74},
  year={2007},
  organization={IEEE}
}

@inproceedings{mulloni2011handheld,
  title={Handheld augmented reality indoor navigation with activity-based instructions},
  author={Mulloni, Alessandro and Seichter, Hartmut and Schmalstieg, Dieter},
  booktitle={Proceedings of the 13th international conference on human computer interaction with mobile devices and services},
  pages={211--220},
  year={2011}
}

@inproceedings{kallwies2020determining,
  title={Determining and improving the localization accuracy of AprilTag detection},
  author={Kallwies, Jan and Forkel, Bianca and Wuensche, Hans-Joachim},
  booktitle={2020 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={8288--8294},
  year={2020},
  organization={IEEE}
}

@inproceedings{wang2016apriltag,
  title={AprilTag 2: Efficient and robust fiducial detection},
  author={Wang, John and Olson, Edwin},
  booktitle={2016 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={4193--4198},
  year={2016},
  organization={IEEE}
}

@inproceedings{zhao2020relative,
  title={Relative Localization for UAVs Based on April-Tags},
  author={Zhao, Boxin and Li, Zongzhe and Jiang, Jun and Zhao, Xiaolin},
  booktitle={2020 Chinese Control And Decision Conference (CCDC)},
  pages={444--449},
  year={2020},
  organization={IEEE}
}

@article{nguyen2021range,
  title={Range-focused fusion of camera-IMU-UWB for accurate and drift-reduced localization},
  author={Nguyen, Thien Hoang and Nguyen, Thien-Minh and Xie, Lihua},
  journal={IEEE Robotics and Automation Letters},
  volume={6},
  number={2},
  pages={1678--1685},
  year={2021},
  publisher={IEEE}
}

@inproceedings{olsson2014cooperative,
  title={Cooperative localization using a foot-mounted inertial navigation system and ultrawideband ranging},
  author={Olsson, Fredrik and Rantakokko, Jouni and Nyg{\aa}rds, Jonas},
  booktitle={2014 International conference on indoor positioning and indoor navigation (IPIN)},
  pages={122--131},
  year={2014},
  organization={IEEE}
}

@article{shule2020uwb,
  title={Uwb-based localization for multi-uav systems and collaborative heterogeneous multi-robot systems},
  author={Shule, Wang and Almansa, Carmen Mart{\'\i}nez and Queralta, Jorge Pe{\~n}a and Zou, Zhuo and Westerlund, Tomi},
  journal={Procedia Computer Science},
  volume={175},
  pages={357--364},
  year={2020},
  publisher={Elsevier}
}

@article{vcapkun2002gps,
  title={GPS-free positioning in mobile ad hoc networks},
  author={{\v{C}}apkun, Srdjan and Hamdi, Maher and Hubaux, Jean-Pierre},
  journal={Cluster Computing},
  volume={5},
  pages={157--167},
  year={2002},
  publisher={Springer}
}

@inproceedings{shao2018marble,
  title={Marble: Mobile augmented reality using a distributed ble beacon infrastructure},
  author={Shao, Chong and Islam, Bashima and Nirjon, Shahriar},
  booktitle={2018 IEEE/ACM Third International Conference on Internet-of-Things Design and Implementation (IoTDI)},
  pages={60--71},
  year={2018},
  organization={IEEE}
}

@inproceedings{gomez2013indoor,
  title={Indoor augmented reality based on ultrasound localization systems},
  author={G{\'o}mez, David and Tarr{\'\i}o, Paula and Li, Juan and Bernardos, Ana M and Casar, Jos{\'e} R},
  booktitle={Highlights on Practical Applications of Agents and Multi-Agent Systems: International Workshops of PAAMS 2013, Salamanca, Spain, May 22-24, 2013. Proceedings 11},
  pages={202--212},
  year={2013},
  organization={Springer}
}

@inproceedings{lazik2015alps,
  title={ALPS: A bluetooth and ultrasound platform for mapping and localization},
  author={Lazik, Patrick and Rajagopal, Niranjini and Shih, Oliver and Sinopoli, Bruno and Rowe, Anthony},
  booktitle={Proceedings of the 13th ACM conference on embedded networked sensor systems},
  pages={73--84},
  year={2015}
}

@inproceedings{li2018automatic,
  title={An automatic and accurate localization system for firefighters},
  author={Li, Jinyang and Xie, Zhiheng and Sun, Xiaoshan and Tang, Jian and Liu, Hengchang and Stankovic, John A},
  booktitle={2018 IEEE/ACM Third International Conference on Internet-of-Things Design and Implementation (IoTDI)},
  pages={13--24},
  year={2018},
  organization={IEEE}
}

@inproceedings{dhekne2019trackio,
  title={TrackIO: Tracking First Responders Inside-Out.},
  author={Dhekne, Ashutosh and Chakraborty, Ayon and Sundaresan, Karthikeyan and Rangarajan, Sampath},
  booktitle={NSDI},
  volume={19},
  pages={751--764},
  year={2019}
}

@inproceedings{gentner2017simultaneous,
  title={Simultaneous localization and mapping for pedestrians using low-cost ultra-wideband system and gyroscope},
  author={Gentner, Christian and Ulmschneider, Markus},
  booktitle={2017 International Conference on Indoor Positioning and Indoor Navigation (IPIN)},
  pages={1--8},
  year={2017},
  organization={IEEE}
}

@inproceedings{liu2017cooperative,
  title={Cooperative relative positioning of mobile users by fusing IMU inertial and UWB ranging information},
  author={Liu, Ran and Yuen, Chau and Do, Tri-Nhut and Jiao, Dewei and Liu, Xiang and Tan, U-Xuan},
  booktitle={2017 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={5623--5629},
  year={2017},
  organization={IEEE}
}

@inproceedings{rajagopal2019improving,
  title={Improving augmented reality relocalization using beacons and magnetic field maps},
  author={Rajagopal, Niranjini and Miller, John and Kumar, Krishna Kumar Reghu and Luong, Anh and Rowe, Anthony},
  booktitle={2019 International Conference on Indoor Positioning and Indoor Navigation (IPIN)},
  pages={1--8},
  year={2019},
  organization={IEEE}
}

@inproceedings{song2019uwb,
  title={Uwb/lidar fusion for cooperative range-only slam},
  author={Song, Yang and Guan, Mingyang and Tay, Wee Peng and Law, Choi Look and Wen, Changyun},
  booktitle={2019 international conference on robotics and automation (ICRA)},
  pages={6568--6574},
  year={2019},
  organization={IEEE}
}

@inproceedings{wang2017ultra,
  title={Ultra-wideband aided fast localization and mapping system},
  author={Wang, Chen and Zhang, Handuo and Nguyen, Thien-Minh and Xie, Lihua},
  booktitle={2017 IEEE/RSJ international conference on intelligent robots and systems (IROS)},
  pages={1602--1609},
  year={2017},
  organization={IEEE}
}

@inproceedings{nagpal2003organizing,
  title={Organizing a global coordinate system from local information on an ad hoc sensor network},
  author={Nagpal, Radhika and Shrobe, Howard and Bachrach, Jonathan},
  booktitle={Information Processing in Sensor Networks: Second International Workshop, IPSN 2003, Palo Alto, CA, USA, April 22--23, 2003 Proceedings},
  pages={333--348},
  year={2003},
  organization={Springer}
}

@inproceedings{savvides2001dynamic,
  title={Dynamic fine-grained localization in ad-hoc networks of sensors},
  author={Savvides, Andreas and Han, Chih-Chieh and Strivastava, Mani B},
  booktitle={Proceedings of the 7th annual international conference on Mobile computing and networking},
  pages={166--179},
  year={2001}
}

@inproceedings{eren2004rigidity,
  title={Rigidity, computation, and randomization in network localization},
  author={Eren, Tolga and Goldenberg, OK and Whiteley, Walter and Yang, Yang Richard and Morse, A Stephen and Anderson, Brian DO and Belhumeur, Peter N},
  booktitle={IEEE INFOCOM 2004},
  volume={4},
  pages={2673--2684},
  year={2004},
  organization={IEEE}
}

@inproceedings{moore2004robust,
  title={Robust distributed network localization with noisy range measurements},
  author={Moore, David and Leonard, John and Rus, Daniela and Teller, Seth},
  booktitle={Proceedings of the 2nd international conference on Embedded networked sensor systems},
  pages={50--61},
  year={2004}
}

@inproceedings{rad2011cooperative,
  title={Cooperative mobile network localization via subspace tracking},
  author={Rad, Hadi Jamali and Amar, Alon and Leus, Geert},
  booktitle={2011 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={2612--2615},
  year={2011},
  organization={IEEE}
}

@inproceedings{nguyen2020vision,
  title={Vision-based multi-MAV localization with anonymous relative measurements using coupled probabilistic data association filter},
  author={Nguyen, Ty and Mohta, Kartik and Taylor, Camillo J and Kumar, Vijay},
  booktitle={2020 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={3349--3355},
  year={2020},
  organization={IEEE}
}

@article{walter2019uvdar,
  title={Uvdar system for visual relative localization with application to leader--follower formations of multirotor uavs},
  author={Walter, Viktor and Staub, Nicolas and Franchi, Antonio and Saska, Martin},
  journal={IEEE Robotics and Automation Letters},
  volume={4},
  number={3},
  pages={2637--2644},
  year={2019},
  publisher={IEEE}
}

@article{ziegler2021distributed,
  title={Distributed formation estimation via pairwise distance measurements},
  author={Ziegler, Thomas and Karrer, Marco and Schmuck, Patrik and Chli, Margarita},
  journal={IEEE Robotics and Automation Letters},
  volume={6},
  number={2},
  pages={3017--3024},
  year={2021},
  publisher={IEEE}
}

@article{bai2020high,
  title={A high-precision and low-cost IMU-based indoor pedestrian positioning technique},
  author={Bai, Nan and Tian, Yuan and Liu, Ye and Yuan, Zhengxi and Xiao, Zhuoling and Zhou, Jun},
  journal={IEEE Sensors Journal},
  volume={20},
  number={12},
  pages={6716--6726},
  year={2020},
  publisher={IEEE}
}

@inproceedings{cao2021relative,
  title={Relative localization of mobile robots with multiple ultra-wideband ranging measurements},
  author={Cao, Zhiqiang and Liu, Ran and Yuen, Chau and Athukorala, Achala and Ng, Benny Kai Kiat and Mathanraj, Muraleetharan and Tan, U-Xuan},
  booktitle={2021 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={5857--5863},
  year={2021},
  organization={IEEE}
}

@article{guo2019ultra,
  title={Ultra-wideband and odometry-based cooperative relative localization with application to multi-UAV formation control},
  author={Guo, Kexin and Li, Xiuxian and Xie, Lihua},
  journal={IEEE transactions on cybernetics},
  volume={50},
  number={6},
  pages={2590--2603},
  year={2019},
  publisher={IEEE}
}

@article{guo2017ultra,
  title={Ultra-wideband based cooperative relative localization algorithm and experiments for multiple unmanned aerial vehicles in GPS denied environments},
  author={Guo, Kexin and Qiu, Zhirong and Meng, Wei and Xie, Lihua and Teo, Rodney},
  journal={International Journal of Micro Air Vehicles},
  volume={9},
  number={3},
  pages={169--186},
  year={2017},
  publisher={SAGE Publications Sage UK: London, England}
}

@inproceedings{li2020relative,
  title={Relative localization in multi-robot systems based on dead reckoning and uwb ranging},
  author={Li, Ming and Chang, Zhuang and Zhong, Zhen and Gao, Yan},
  booktitle={2020 IEEE 23rd International Conference on Information Fusion (FUSION)},
  pages={1--7},
  year={2020},
  organization={IEEE}
}

@article{xu2022omni,
  title={Omni-Swarm: A Decentralized Omnidirectional Visual--Inertial--UWB State Estimation System for Aerial Swarms},
  author={Xu, Hao and Zhang, Yichen and Zhou, Boyu and Wang, Luqi and Yao, Xinjie and Meng, Guotao and Shen, Shaojie},
  journal={IEEE Transactions on Robotics},
  volume={38},
  number={6},
  pages={3374--3394},
  year={2022},
  publisher={IEEE}
}

@inproceedings{xu2020decentralized,
  title={Decentralized visual-inertial-uwb fusion for relative state estimation of aerial swarm},
  author={Xu, Hao and Wang, Luqi and Zhang, Yichen and Qiu, Kejie and Shen, Shaojie},
  booktitle={2020 IEEE international conference on robotics and automation (ICRA)},
  pages={8776--8782},
  year={2020},
  organization={IEEE}
}

@misc{optitrack,
 title={OptiTrack},
 howpublished = "\url{https://optitrack.com/}",
 journal={OptiTrack},
 note = "Last accessed 12 March 2023"
}

@misc{vicon,
 title={Vicon},
 howpublished = "\url{https://www.vicon.com/}",
 journal={Vicon},
 note = "Last accessed 12 March 2023"
}

@INPROCEEDINGS{5940633,
  author={Taris, T. and Begueret, JB. and Deval, Y.},
  booktitle={2011 IEEE Radio Frequency Integrated Circuits Symposium}, 
  title={A 60µW LNA for 2.4 GHz wireless sensors network applications}, 
  year={2011},
  volume={},
  number={},
  pages={1-4},
  doi={10.1109/RFIC.2011.5940633}}
@misc{HSMS285x,
  author = "Hewlett-Packards",

  howpublished = "\url{https://www.hpl.hp.com/hpjournal/95dec/dec95a12.pdf}",
}
@INPROCEEDINGS{4523148,
  author={van Elzakker, Michiel and van Tuijl, Ed and Geraedts, Paul and Schinkel, Daniel and Klumperink, Eric and Nauta, Bram},
  booktitle={2008 IEEE International Solid-State Circuits Conference - Digest of Technical Papers}, 
  title={A 1.9μW 4.4fJ/Conversion-step 10b 1MS/s Charge-Redistribution ADC}, 
  year={2008},
  volume={},
  number={},
  pages={244-610},
  doi={10.1109/ISSCC.2008.4523148}}

@misc{OpenStreetMap,
   author = {{OpenStreetMap contributors}},
   title = {{OpenStreetMap}},
   howpublished = "\url{https://www.openstreetmap.org}",
   year = {2024},
 }


@article{ibrahim2011cellsense,
  title={CellSense: An accurate energy-efficient GSM positioning system},
  author={Ibrahim, Mohamed and Youssef, Moustafa},
  journal={IEEE Transactions on Vehicular Technology},
  volume={61},
  number={1},
  pages={286--296},
  year={2011},
  publisher={IEEE}
}
@inproceedings{ibrahim2011hidden,
  title={A hidden markov model for localization using low-end GSM cell phones},
  author={Ibrahim, Mohamed and Youssef, Moustafa},
  booktitle={2011 IEEE International Conference on Communications (ICC)},
  pages={1--5},
  year={2011},
  organization={IEEE}
}
@inproceedings{paek2011energy,
  title={Energy-efficient positioning for smartphones using cell-id sequence matching},
  author={Paek, Jeongyeup and Kim, Kyu-Han and Singh, Jatinder P and Govindan, Ramesh},
  booktitle={Proceedings of the 9th international conference on Mobile systems, applications, and services},
  pages={293--306},
  year={2011}
}
@inproceedings{sallouha2017localization,
  title={Localization in long-range ultra narrow band IoT networks using RSSI},
  author={Sallouha, Hazem and Chiumento, Alessandro and Pollin, Sofie},
  booktitle={2017 IEEE International Conference on Communications (ICC)},
  pages={1--6},
  year={2017},
  organization={IEEE}
}
@inproceedings{inproceedings,
author = {Yang, Jie and Varshavsky, Alexander and Liu, Hongbo and Chen, Yingying and Gruteser, Marco},
year = {2010},
month = {09},
pages = {223-226},
title = {Accuracy Characterization of Cell Tower Localization},
doi = {10.1145/1864349.1864384}
}
@article{acedo2018analysis,
  title={Analysis of the influence of PCI planning on the physical uplink control channel in LTE},
  author={Acedo-Hern{\'a}ndez, Roc{\'\i}o and Toril, Mat{\'\i}as and Luna-Ram{\'\i}rez, Salvador and Fern{\'a}ndez-Segovia, Jos{\'e} A and {\'U}beda, Carlos},
  journal={Wireless Personal Communications},
  volume={98},
  pages={629--649},
  year={2018},
  publisher={Springer}
}
@article{acedo2017pci,
  title={A PCI planning algorithm for jointly reducing reference signal collisions in LTE uplink and downlink},
  author={Acedo-Hern{\'a}ndez, Roc{\'\i}o and Toril, Matias and Luna-Ram{\'\i}rez, Salvador and Ubeda, Carlos},
  journal={Computer Networks},
  volume={119},
  pages={112--123},
  year={2017},
  publisher={Elsevier}
}
@book{sesia2011lte,
  title={LTE-the UMTS long term evolution: from theory to practice},
  author={Sesia, Stefania and Toufik, Issam and Baker, Matthew},
  year={2011},
  publisher={John Wiley \& Sons}
}
@article{zhang2014some,
  title={Some New Results on the Cross Correlation of $ m $-sequences},
  author={Zhang, Tao and Li, Shuxing and Feng, Tao and Ge, Gennian},
  journal={IEEE transactions on information theory},
  volume={60},
  number={5},
  pages={3062--3068},
  year={2014},
  publisher={IEEE}
}
@inproceedings{yang2010accuracy,
  title={Accuracy characterization of cell tower localization},
  author={Yang, Jie and Varshavsky, Alexander and Liu, Hongbo and Chen, Yingying and Gruteser, Marco},
  booktitle={Proceedings of the 12th ACM international conference on Ubiquitous computing},
  pages={223--226},
  year={2010}
}
@inproceedings{laitinen2001database,
  title={Database correlation method for GSM location},
  author={Laitinen, Heikki and Lahteenmaki, Jaakko and Nordstrom, Tero},
  booktitle={IEEE VTS 53rd Vehicular Technology Conference, Spring 2001. Proceedings (Cat. No. 01CH37202)},
  volume={4},
  pages={2504--2508},
  year={2001},
  organization={IEEE}
}
@article{ergen2013rssi,
  title={RSSI-fingerprinting-based mobile phone localization with route constraints},
  author={Ergen, Sinem Coleri and Tetikol, Huseyin Serhat and Kontik, Mehmet and Sevlian, Raffi and Rajagopal, Ram and Varaiya, Pravin},
  journal={IEEE Transactions on Vehicular Technology},
  volume={63},
  number={1},
  pages={423--428},
  year={2013},
  publisher={IEEE}
}
@inproceedings{chakraborty2015network,
  title={Network-side positioning of cellular-band devices with minimal effort},
  author={Chakraborty, Ayon and Ortiz, Luis E and Das, Samir R},
  booktitle={2015 IEEE Conference on Computer Communications (INFOCOM)},
  pages={2767--2775},
  year={2015},
  organization={IEEE}
}
@inproceedings{yi2021cellular,
  title={Cellular-assisted COVID-19 contact tracing},
  author={Yi, Fan and Xie, Yaxiong and Jamieson, Kyle},
  booktitle={Proceedings of the 2nd Workshop on Deep Learning for Wellbeing Applications Leveraging Mobile Devices and Edge Computing},
  pages={1--6},
  year={2021}
}
@inproceedings{zhu2023experience,
  title={Experience: Large-scale Cellular Localization for Pickup Position Recommendation at Black-hole},
  author={Zhu, Shuli and Li, Lingkun and Wang, Xuyu and Liu, Changcheng and Jiang, Yuqin and Huo, Zengwei and Chai, Hua and Liu, Jiqiang and Tao, Dan and Gao, Ruipeng},
  booktitle={Proceedings of the 29th Annual International Conference on Mobile Computing and Networking},
  pages={1--15},
  year={2023}
}
@INPROCEEDINGS{8411262,
  author={Luo, Shixin and Ng, Yibin and Lim, Terence Zheng Wei and Tan, Cliff Choon Hua and He, Nannan and Manai, Giuseppe and Li, Ying},
  booktitle={2018 19th IEEE International Conference on Mobile Data Management (MDM)}, 
  title={Improved Localisation Using Spatio-Temporal Data from Cellular Network}, 
  year={2018},
  volume={},
  number={},
  pages={56-65},
  keywords={Global Positioning System;Poles and towers;Mobile handsets;Oscillators;Cellular networks;Data mining;Business;cellular networks;localisation;spatio temporal data},
  doi={10.1109/MDM.2018.00022}}
@inproceedings {266949,
author = {Arvind Thiagarajan and Lenin Ravindranath and Hari Balakrishnan and Samuel Madden and Lewis Girod},
title = {Accurate, {Low-Energy} Trajectory Mapping for Mobile Devices},
booktitle = {8th USENIX Symposium on Networked Systems Design and Implementation (NSDI 11)},
year = {2011},
address = {Boston, MA},
url = {https://www.usenix.org/conference/nsdi11/accurate-low-energy-trajectory-mapping-mobile-devices},
publisher = {USENIX Association},
month = mar
}
@inproceedings{spirito2001experimental,
  title={Experimental performance of methods to estimate the location of legacy handsets in GSM},
  author={Spirito, Maurizio A and Poykko, Sami and Knuuttila, Olli},
  booktitle={IEEE 54th Vehicular Technology Conference. VTC Fall 2001. Proceedings (Cat. No. 01CH37211)},
  volume={4},
  pages={2716--2720},
  year={2001},
  organization={IEEE}
}
@article{lin2005mobile,
  title={Mobile location estimation based on differences of signal attenuations for GSM systems},
  author={Lin, Ding-Bing and Juang, Rong-Terng},
  journal={IEEE transactions on vehicular technology},
  volume={54},
  number={4},
  pages={1447--1454},
  year={2005},
  publisher={IEEE}
}
@article{del2017survey,
  title={Survey of cellular mobile radio localization methods: From 1G to 5G},
  author={del Peral-Rosado, Jos{\'e} A and Raulefs, Ronald and L{\'o}pez-Salcedo, Jos{\'e} A and Seco-Granados, Gonzalo},
  journal={IEEE Communications Surveys \& Tutorials},
  volume={20},
  number={2},
  pages={1124--1148},
  year={2017},
  publisher={IEEE}
}
@article{xu2016maximum,
  title={Maximum likelihood TOA and OTDOA estimation with first arriving path detection for 3GPP LTE system},
  author={Xu, Wen and Huang, Ming and Zhu, Chen and Dammann, Armin},
  journal={Transactions on Emerging Telecommunications Technologies},
  volume={27},
  number={3},
  pages={339--356},
  year={2016},
  publisher={Wiley Online Library}
}
@inproceedings{del2015floor,
  title={Floor detection with indoor vertical positioning in LTE femtocell networks},
  author={del Peral-Rosado, Jos{\'e} A and Bavaro, Michele and L{\'o}pez-Salcedo, Jos{\'e} A and Seco-Granados, Gonzalo and Chawdhry, Pravir and Fortuny-Guasch, Joaquim and Crosta, Paolo and Zanier, Francesca and Crisci, Massimo},
  booktitle={2015 IEEE Globecom Workshops (GC Wkshps)},
  pages={1--6},
  year={2015},
  organization={IEEE}
}
@article{pecoraro2018csi,
  title={CSI-based fingerprinting for indoor localization using LTE signals},
  author={Pecoraro, Giovanni and Di Domenico, Simone and Cianca, Ernestina and De Sanctis, Mauro},
  journal={EURASIP Journal on Advances in Signal Processing},
  volume={2018},
  pages={1--18},
  year={2018},
  publisher={Springer}
}
@inproceedings{garg2023sirius,
  title={Sirius: A self-localization system for resource-constrained iot sensors},
  author={Garg, Nakul and Roy, Nirupam},
  booktitle={Proceedings of the 21st Annual International Conference on Mobile Systems, Applications and Services},
  pages={289--302},
  year={2023}
}
@inproceedings{iyer2019living,
  title={Living IoT: A flying wireless platform on live insects},
  author={Iyer, Vikram and Nandakumar, Rajalakshmi and Wang, Anran and Fuller, Sawyer B and Gollakota, Shyamnath},
  booktitle={The 25th Annual International Conference on Mobile Computing and Networking},
  pages={1--15},
  year={2019}
}
@inproceedings{xiong2013arraytrack,
  title={$\{$ArrayTrack$\}$: A $\{$Fine-Grained$\}$ indoor location system},
  author={Xiong, Jie and Jamieson, Kyle},
  booktitle={10th USENIX Symposium on Networked Systems Design and Implementation (NSDI 13)},
  pages={71--84},
  year={2013}
}
@article{fischer2014observed,
  title={Observed time difference of arrival (OTDOA) positioning in 3GPP LTE},
  author={Fischer, Sven},
  journal={Qualcomm White Pap},
  volume={1},
  number={1},
  pages={1--62},
  year={2014}
}
@INPROCEEDINGS{8485819,
  author={Palacios, Joan and Bielsa, Guillermo and Casari, Paolo and Widmer, Joerg},
  booktitle={IEEE INFOCOM 2018 - IEEE Conference on Computer Communications}, 
  title={Communication-Driven Localization and Mapping for Millimeter Wave Networks}, 
  year={2018},
  volume={},
  number={},
  pages={2402-2410},
  keywords={Shape;Simultaneous localization and mapping;Training;Estimation;Standards;Shape measurement;Handover},
  doi={10.1109/INFOCOM.2018.8485819}}

@inproceedings{palacios2017jade,
  title={JADE: Zero-knowledge device localization and environment mapping for millimeter wave systems},
  author={Palacios, Joan and Casari, Paolo and Widmer, Joerg},
  booktitle={IEEE INFOCOM 2017-IEEE Conference on Computer Communications},
  pages={1--9},
  year={2017},
  organization={IEEE}
}
@article{lv2019envelope,
  title={Envelope detection of 16QAM single carrier signal for IM/DD RoF system at Q-band},
  author={Lv, Kai and Pan, Xiaolong and Zhang, Junwen and Wang, Kaihui and Guo, Dong and Zhang, Qi and Deng, ao Li and Xin, Xiangjun},
  journal={IEICE Electronics Express},
  volume={16},
  number={4},
  pages={20180986--20180986},
  year={2019},
  publisher={The Institute of Electronics, Information and Communication Engineers}
}
@inproceedings{li2015w,
  title={W-band OFDM RoF system with simple envelope detector down-conversion},
  author={Li, Che-Hao and Wu, Meng-Fan and Lin, Chi-Hsiang and Lin, Chun-Ting},
  booktitle={Optical Fiber Communication Conference},
  pages={W4G--6},
  year={2015},
  organization={Optica Publishing Group}
}
@online{QRPWebsite,
  title = {Ultimate Transceiver Kit},
  url = {http://qrp.gr/ultimatextalset/index.htm},
  note = {Accessed: \today}
}
@online{EEEGuideSquareLawDiodeModulator,
  title = {Square Law Diode Modulator},
  author = {Author (if available)},
  year = {Publication Year (if available)},
  url = {https://www.eeeguide.com/square-law-diode-modulator/},
  note = {Accessed: \today}
}
@inproceedings{rostami2021mixiq,
  title={MIXIQ: re-thinking ultra-low power receiver design for next-generation on-body applications},
  author={Rostami, Mohammad and Chen, Xingda and Feng, Yuda and Sundaresan, Karthikeyan and Ganesan, Deepak},
  booktitle={Proceedings of the 27th Annual International Conference on Mobile Computing and Networking},
  pages={364--377},
  year={2021}
}
@inproceedings{ensworth2017low,
  title={A low power 2.4 GHz superheterodyne receiver architecture with external LO for wirelessly powered backscatter tags and sensors},
  author={Ensworth, Joshua F and Hoang, Alexander T and Reynolds, Matthew S},
  booktitle={2017 IEEE International Conference on RFID (RFID)},
  pages={149--154},
  year={2017},
  organization={IEEE}
}
@inproceedings{perez2018battery,
  title={Battery-Free 802.15. 4 Receiver},
  author={P{\'e}rez-Penichet, Carlos and Noda, Claro and Varshney, Ambuj and Voigt, Thiemo},
  booktitle={2018 17th ACM/IEEE International Conference on Information Processing in Sensor Networks (IPSN)},
  pages={164--175},
  year={2018},
  organization={IEEE}
}

@inproceedings{galisteo2020two,
  title={Two to tango: Hybrid light and backscatter networks for next billion devices},
  author={Galisteo, Ander and Varshney, Ambuj and Giustiniano, Domenico},
  booktitle={Proceedings of the 18th International Conference on Mobile Systems, Applications, and Services},
  pages={80--93},
  year={2020}
}
@inproceedings{li2022passive,
  title={Passive $\{$DSSS$\}$: Empowering the downlink communication for backscatter systems},
  author={Li, Songfan and Zheng, Hui and Zhang, Chong and Song, Yihang and Yang, Shen and Chen, Minghua and Lu, Li and Li, Mo},
  booktitle={19th USENIX Symposium on Networked Systems Design and Implementation (NSDI 22)},
  pages={913--928},
  year={2022}
}
@inproceedings{jog2022enabling,
  title={Enabling $\{$IoT$\}$$\{$Self-Localization$\}$ Using Ambient 5G Signals},
  author={Jog, Suraj and Guan, Junfeng and Madani, Sohrab and Lu, Ruochen and Gong, Songbin and Vasisht, Deepak and Hassanieh, Haitham},
  booktitle={19th USENIX Symposium on Networked Systems Design and Implementation (NSDI 22)},
  pages={1011--1026},
  year={2022}
}
@inproceedings{guan2021efficient,
  title={Efficient Wideband Spectrum Sensing Using $\{$MEMS$\}$ Acoustic Resonators},
  author={Guan, Junfeng and Zhang, Jitian and Lu, Ruochen and Seo, Hyungjoo and Zhou, Jin and Gong, Songbin and Hassanieh, Haitham},
  booktitle={18th USENIX Symposium on Networked Systems Design and Implementation (NSDI 21)},
  pages={809--825},
  year={2021}
}
@article{westervelt1951theory,
  title={The theory of steady forces caused by sound waves},
  author={Westervelt, Peter J},
  journal={The Journal of the Acoustical Society of America},
  volume={23},
  number={3},
  pages={312--315},
  year={1951},
  publisher={Acoustical Society of America}
}
@article{westervelt1957scattering,
  title={Scattering of sound by sound},
  author={Westervelt, Peter J},
  journal={The Journal of the Acoustical Society of America},
  volume={29},
  number={2},
  pages={199--203},
  year={1957},
  publisher={Acoustical Society of America}
}
@inproceedings{vasisht2018body,
  title={In-body backscatter communication and localization},
  author={Vasisht, Deepak and Zhang, Guo and Abari, Omid and Lu, Hsiao-Ming and Flanz, Jacob and Katabi, Dina},
  booktitle={Proceedings of the 2018 Conference of the ACM Special Interest Group on Data Communication},
  pages={132--146},
  year={2018}
}
@article{gomes2009rfid,
  title={RFID for location proposes based on the intermodulation distortion},
  author={Gomes, Hugo and Carvalho, Nuno Borges},
  journal={Sensors \& Transducers},
  volume={106},
  number={7},
  pages={85},
  year={2009},
  publisher={IFSA Publishing, SL}
}
@inproceedings{gomes2007use,
  title={The use of intermodulation distortion for the design of passive RFID},
  author={Gomes, Hugo Cravo and Carvalho, Nuno Borges},
  booktitle={2007 European Radar Conference},
  pages={377--380},
  year={2007},
  organization={IEEE}
}
@article{rasilainen2014design,
  title={On design and evaluation of harmonic transponders},
  author={Rasilainen, Kimmo and Ilvonen, Janne and Lehtovuori, Anu and Hannula, Jari-Matti and Viikari, Ville},
  journal={IEEE Transactions on Antennas and Propagation},
  volume={63},
  number={1},
  pages={15--23},
  year={2014},
  publisher={IEEE}
}
@article{colpitts2004harmonic,
  title={Harmonic radar transceiver design: Miniature tags for insect tracking},
  author={Colpitts, Bruce G and Boiteau, Gilles},
  journal={IEEE Transactions on Antennas and Propagation},
  volume={52},
  number={11},
  pages={2825--2832},
  year={2004},
  publisher={IEEE}
}
@inproceedings{roy2017backdoor,
  title={Backdoor: Making microphones hear inaudible sounds},
  author={Roy, Nirupam and Hassanieh, Haitham and Roy Choudhury, Romit},
  booktitle={Proceedings of the 15th Annual International Conference on Mobile Systems, Applications, and Services},
  pages={2--14},
  year={2017}
}
@article{hsiao2018passive,
  title={A passive RFID-based location system for personnel and asset monitoring},
  author={Hsiao, Rong-Shue and Kao, Chun-Hao and Chen, Tian-Xiang and Chen, Jui-Lun},
  journal={Technology and Health Care},
  volume={26},
  number={1},
  pages={11--16},
  year={2018},
  publisher={IOS Press}
}
@INPROCEEDINGS{10154401,
  author={Rodrigues, Bruno and Scheid, Eder J. and Willems, Julius and Stiller, Burkhard},
  booktitle={NOMS 2023-2023 IEEE/IFIP Network Operations and Management Symposium}, 
  title={Real-time Medical Devices Inventory Tracking – a Hands-on Experience}, 
  year={2023},
  volume={},
  number={},
  pages={1-6},
  keywords={Medical devices;Hospitals;Pandemics;Logic gates;Fingerprint recognition;Real-time systems;Smart phones;Indoor Tracking;Inventory;Bluetooth Low Energy (BLE);COVID-19;Healthcare},
  doi={10.1109/NOMS56928.2023.10154401}}
@article{oztekin2010rfid,
  title={An RFID network design methodology for asset tracking in healthcare},
  author={Oztekin, Asil and Pajouh, Foad M and Delen, Dursun and Swim, Leva K},
  journal={Decision support systems},
  volume={49},
  number={1},
  pages={100--109},
  year={2010},
  publisher={Elsevier}
}
@article{bendavid2010redesigning,
  title={Redesigning the replenishment process of medical supplies in hospitals with RFID},
  author={Bendavid, Ygal and Boeck, Harold and Philippe, Richard},
  journal={Business Process Management Journal},
  volume={16},
  number={6},
  pages={991--1013},
  year={2010},
  publisher={Emerald Group Publishing Limited}
}
@inproceedings{balakrishnan2009efficient,
  title={Efficient geo-tracking and adaptive routing of mobile assets},
  author={Balakrishnan, Dineshbalu and Nayak, Amiya and Dhar, Pulak and Kaul, Shailesh},
  booktitle={2009 11th IEEE International Conference on High Performance Computing and Communications},
  pages={289--296},
  year={2009},
  organization={IEEE}
}
@inproceedings{manoharan2009gps,
  title={On GPS tracking of mobile devices},
  author={Manoharan, Sathiamoorthy},
  booktitle={2009 Fifth International Conference on Networking and Services},
  pages={415--418},
  year={2009},
  organization={IEEE}
}
@inproceedings{bilgic2011secure,
  title={A secure tracking system for GPS-enabled mobile phones},
  author={Bilgic, Hasan Tahsin and Alkar, Ali Ziya},
  booktitle={ICIMU 2011: Proceedings of the 5th international Conference on Information Technology \& Multimedia},
  pages={1--5},
  year={2011},
  organization={IEEE}
}
@article{parrino2021lopatran,
  title={Lopatran: Low power asset tracking by means of narrow band iot (nb-iot) technology},
  author={Parrino, Stefano and Peruzzi, Giacomo and Pozzebon, Alessandro},
  journal={Sensors},
  volume={21},
  number={11},
  pages={3772},
  year={2021},
  publisher={MDPI}
}
@inproceedings{suryani2020narrowband,
  title={Narrowband-IoT network for asset tracking system},
  author={Suryani, V and Wardana, AA and others},
  booktitle={IOP Conference Series: Materials Science and Engineering},
  volume={830},
  number={2},
  pages={022087},
  year={2020},
  organization={IOP Publishing}
}
@online{powerfleet,
  author = {PowerFleet},
  title = {Asset Tracking Solutions},
  year = {Year},
  url = {https://www.powerfleet.com/asset-tracking/},
  note = {Accessed: Month Day, Year}
}
@online{digitalmatter,
  author = {Digital Matter},
  title = {Cold Chain Monitoring},
  year = {Year},
  url = {https://www.digitalmatter.com/applications/cold-chain-monitoring/},
  note = {Accessed: Month Day, Year}
}
@online{hanhaa,
  author = {Hanhaa},
  title = {Cold Chain Monitoring},
  year = {Year},
  url = {https://hanhaa.com/cold-chain/},
  note = {Accessed: Month Day, Year}
}
@inproceedings{kavlak2012pci,
  title={PCI planning strategies for long term evolution networks},
  author={Kavlak, Hakan and Ilk, Hakki},
  booktitle={NETWORKING 2012 Workshops: International IFIP TC 6 Workshops, ETICS, HetsNets, and CompNets, Held at NETWORKING 2012, Prague, Czech Republic, May 25, 2012. Proceedings 11},
  pages={151--156},
  year={2012},
  organization={Springer}
}
